Compact and Efficient KEMs over NTRU Lattices

The NTRU lattice is a promising candidate to construct practical cryptosystems, in particular key encapsulation mechanism (KEM), resistant to quantum computing attacks. Nevertheless, there are still some inherent obstacles to NTRU-based KEM schemes in having integrated performance, taking security, bandwidth, error probability, and computational efficiency \emph{as a whole}, that is as good as and even better than their \{R,M\}LWE-based counterparts. In this work, we solve this problem by presenting a new family of NTRU-based KEM schemes, referred to as CTRU and CNTR. By bridging low-dimensional lattice codes and high-dimensional NTRU-lattice-based cryptography with careful design and analysis, to the best of our knowledge CTRU and CNTR are the first NTRU-based KEM schemes with scalable ciphertext compression via only one \emph{single} ciphertext polynomial, and are the first that could outperform \{R,M\}LWE-based KEM schemes in integrated performance. For instance, compared to Kyber that is currently the only standardized KEM by NIST, on the recommended parameter set CNTR-768 has about $12\%$ smaller ciphertext size while encapsulating 384-bit keys compared to the fixed 256-bit key size of Kyber, security strengthened by $(8,7)$ bits for classical and quantum security respectively, and significantly lower error probability ($2^{-230}$ of CNTR-768 vs. $2^{-164}$ of Kyber-768). In comparison with the state-of-the-art AVX2 implementation of Kyber-768, CNTR-768 is faster by 1.9X in KeyGen, 2.6X in Encaps, and 1.2X in Decaps, respectively. When compared to the NIST Round 3 finalist NTRU-HRSS, our CNTR-768 has about $15\%$ smaller ciphertext size, and the security is strengthened by $(55,49)$ bits for classical and quantum security respectively. As for the AVX2 implementation, CNTR-768 is faster than NTRU-HRSS by 19X in KeyGen, 2.3X in Encaps, and 1.6X in Decaps, respectively.

==> table/tab-benchmark-of-rlwr-variant-and-saber.tex <==
\begin{table}[H]
%	\scriptsize
	\centering
	\setlength{\tabcolsep}{4.3mm}
	\caption{CPU cycles of CNTR and Saber (in kilo cycles).}
	\begin{tabular}{cccc}
		\hline
		                      Schemes                       & KeyGen & Encaps & Decaps \\ \hline
		             \multirow{1}{*}{CNTR-768}              & 128.5  &  71.2  & 149.7  \\
		\multirow{1}{*}{Saber-768~\cite{saber-nist-round3}} &  94.7  & 109.7  & 138.9  \\ \hline
	\end{tabular}
	\label{tab-benchmark-of-rlwr-variant-and-saber}
\end{table}	

==> table/tab-benchmark-of-saber.tex <==
\begin{table}[H]
%	\scriptsize
	\centering
	\setlength{\tabcolsep}{4.3mm}
	\caption{CPU cycles of CTRU and Saber (in kilo cycles).}
	\begin{tabular}{cccc}
		\hline
		                      Schemes                       & KeyGen & Encaps & Decaps \\ \hline
		             \multirow{1}{*}{CTRU-768}              & 127.2  &  70.1  & 149.2  \\
		\multirow{1}{*}{Saber-768~\cite{saber-nist-round3}} &  94.7  & 109.7  & 138.9  \\ \hline
	\end{tabular}
	\label{tab-benchmark-of-saber}
\end{table}	

==> table/tab-comparisons-rlwr-variant-and-saber.tex <==
\begin{table*}
%	\scriptsize
%	\footnotesize
	\centering
	\setlength{\tabcolsep}{2.2mm}
	\caption{Comparison between CNTR and Saber. The column ``Assumptions'' refers to the underlying hardness assumptions. The column ``Reduction'' means that IND-CCA security is reduced to what kinds of CPA security, where ``IND'' refers to indistinguishability  and ``RPKE'' refers to randomized public-key encryptions. ``Rings'' refers to the underlying polynomial rings. The column ``$n$'' means the total dimension of algebraically structured lattices. ``$q$'' is the modulus. The public key sizes $|pk|$, ciphertext sizes $|ct|$, and B.W. (bandwidth, $|pk|+|ct|$)  are measured in bytes.  ``Sec.C'' and ``Sec.Q'' mean the estimated security expressed in bits in the classical and quantum setting respectively, which are gotten by the same methodology and scripts provided by NTRU KEM and Saber in NIST PQC Round 3, where we  minimize the target values if the two hardness problems, say NTRU and RLWR, have different security values. The column ``$\delta$'' indicates the error probabilities. } 
	\begin{tabular}{ccccccccccc}
		\hline
		                    Schemes                     &                Assumptions                 &                  Reduction                   &                                  Rings                                  & $n$  & $q$  & $|pk|$ & $|ct|$ & B.W. & (Sec.C, Sec.Q) &  $\delta$  \\ \hline
		         \multirow{3}{*}{CNTR (Ours)}           & \multirow{3}{*}{\makecell[c]{NTRU,\\RLWR}} & \multirow{3}{*}{\makecell[c]{IND-CPA\\RPKE}} &          \multirow{3}{*}{$\mathbb{Z}_q[x]/(x^{n}-x^{n/2}+1)$}           & 512  & 3457 &  768   &  640   & 1408 &   (127,115)    & $2^{-153}$ \\
		                                                &                                            &                                              &                                                                         & 768  & 3457 &  1152  &  960   & 2112 &   (191,173)    & $2^{-209}$ \\
		                                                &                                            &                                              &                                                                         & 1024 & 3457 &  1536  &  1280  & 2816 &   (253,230)    & $2^{-264}$ \\ \hline
		\multirow{3}{*}{Saber~\cite{saber-nist-round3}} &           \multirow{3}{*}{MLWR}            & \multirow{3}{*}{\makecell[c]{IND-CPA\\RPKE}} & \multirow{3}{*}{\makecell[c]{$\mathbb{Z}_q[x]/(x^{n/k}+1)$\\$k=2,3,4$}} & 512  & 8192 &  672   &  736   & 1408 &   (118,107)    & $2^{-120}$ \\
		                                                &                                            &                                              &                                                                         & 768  & 8192 &  992   &  1088  & 2080 &   (189,172)    & $2^{-136}$ \\
		                                                &                                            &                                              &                                                                         & 1024 & 8192 &  1312  &  1472  & 2784 &   (260,236)    & $2^{-165}$ \\ \hline
	\end{tabular}
	\label{tab-comparisons-rlwr-variant-and-saber}
\end{table*}	

==> table/tab-comparisons-with-saber.tex <==
\begin{table*}
%	\scriptsize
%	\footnotesize
	\centering
	\setlength{\tabcolsep}{1.5mm}
	\caption{Comparison between CTRU and Saber.} 
	\begin{tabular}{ccccccccccc}
		\hline
		                    Schemes                     &                Assumptions                 &                  Reduction                   &                                  Rings                                  & $n$  & $q$  & $|pk|$ & $|ct|$ & B.W. & (Sec.C, Sec.Q) &  $\delta$  \\ \hline
		         \multirow{3}{*}{CTRU (Ours)}           & \multirow{3}{*}{\makecell[c]{NTRU,\\RLWE}} & \multirow{3}{*}{\makecell[c]{IND-CPA\\RPKE}} &          \multirow{3}{*}{$\mathbb{Z}_q[x]/(x^{n}-x^{n/2}+1)$}           & 512  & 3457 &  768   &  640   & 1408 &   (118,107)    & $2^{-129}$ \\
		                                                &                                            &                                              &                                                                         & 768  & 3457 &  1152  &  960   & 2112 &   (181,164)    & $2^{-166}$ \\
		                                                &                                            &                                              &                                                                         & 1024 & 3457 &  1536  &  1408  & 2944 &   (255,231)    & $2^{-176}$ \\ \hline
		\multirow{3}{*}{Saber~\cite{saber-nist-round3}} &           \multirow{3}{*}{MLWR}            & \multirow{3}{*}{\makecell[c]{IND-CPA\\RPKE}} & \multirow{3}{*}{\makecell[c]{$\mathbb{Z}_q[x]/(x^{n/k}+1)$\\$k=2,3,4$}} & 512  & 8192 &  672   &  736   & 1408 &   (118,107)    & $2^{-120}$ \\
		                                                &                                            &                                              &                                                                         & 768  & 8192 &  992   &  1088  & 2080 &   (189,172)    & $2^{-136}$ \\
		                                                &                                            &                                              &                                                                         & 1024 & 8192 &  1312  &  1472  & 2784 &   (260,236)    & $2^{-165}$ \\ \hline
	\end{tabular}
	\label{tab-comparisons-with-saber}
\end{table*}	
